An Introduction to OFDM-OQAM

The Filter Bank MultiCarrier (FBMC) modulation with Offset QAM (OQAM), also know as OFDM-OQAM, has been very well studied in, roughly speaking, the last 15 years. A rich literature exists on the principle itself, discrete-time version and implementation, equalization, extension to MIMO, etc. This text, written in a tutorial style, explains the idea of Offset QAM and why it works from a Communications Engineer point of view. The language is very simple and the math elementary. Students and researchers in universities or practitioners who are interested in gaining an intuition into the logic behind OFDM-OQAM will hopefully enjoy reading this text. On the other hand, those interested in a quick understanding of the idea, just enough to start using the waveform, can find far better material.

==> PA.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{tikz}
%
%\tikzstyle{axis-line}=[thick, ->, >=stealth]
%\tikzstyle{axis-tick}=[thin]
%\tikzstyle{arrow} = [thick,->]
%
%\begin{document}
%\begin{figure}
%\centering
\begin{tikzpicture}[scale=1]
\draw [axis-line] (-2.5,0) -- (2.5,0) node[below] {$v_i(t)$};
\draw [axis-line] (0,-2.5) -- (0,2.5) node[anchor=east] {$v_o(t)$};

\draw [blue] (-2.3,-2) -- (-1.2,-2) -- (1.2,2) -- (2.3,2);

\end{tikzpicture}
%\caption{bla bla bla}
%\end{figure}
%
% 
%
%\end{document}

